Automation Configuration in Smart Home Systems: Challenges and Opportunities

As the innovation of smart devices and internet-of-things (IoT), smart homes have become prevalent. People tend to transform residences into smart homes by customizing off-the-shelf smart home platforms, instead of creating IoT systems from scratch. Among the alternatives, Home Assistant (HA) is one of the most popular platforms. It allows end-users (i.e., home residents) to smartify homes by (S1) integrating selected devices into the system, and (S2) creating YAML files to control those devices. Unfortunately, due to the diversity of devices and complexity of automatic configurations, many users have difficulty correctly creating YAML files. Consequently, their smart homes may not work as expected, causing frustration and concern in users. This paper presents a novel study on issues of YAML-based automation configuration in smart homes (issues related to S2). We mined the online forum Home Assistant Community for discussion threads related to automation configuration. By manually inspecting 190 threads, we revealed 3 categories of concerns: implementation, optimization, and debugging. Under each category, we classified discussions based on the issue locations and technical concepts involved. Among debugging discussions, we further classified discussions based on users' resolution strategies; we also applied existing analysis tools to buggy YAML files, to assess the tool effectiveness. Our study reveals the common challenges faced by users and frequently applied resolution strategies. There are 129 (68%) examined issues concerning debugging, but existing tools can detect at most 14 issues and fix none. It implies that existing tools provide limited assistance in automation configuration. Our research sheds light on future directions in smart home development.

==> related-original.tex <==
\section{Related Work}

The related work includes empirical studies on Internet-of-Thing (IoT) systems, and automatic bug detection in those systems.
% new tools to detect bugs in such systems.

\subsection{Empirical Studies on IoT Systems}
Studies were recently performed to characterize issues or problems in IoT systems~\cite{fernandes2016security,He2019,alrawi2019sok,Brackenbury2019,Zhou2021,makhshari2021iot,wang2022understanding}. 
For instance, Fernandes et al.~\cite{fernandes2016security} and Alrawi et al.~\cite{alrawi2019sok} analyzed the security properties of IoT systems. Specifically, Fernandes et al.~leveraged static code analysis and testing to reveal design flaws that lead to significant overprivilege in SmartApps. Alrawi et al.~systematically reviewed existing literature on IoT security vulnerabilities, to characterize attack techniques, mitigations, and stakeholders; they also evaluated the security properties of 45 devices by running existing tools. In contrast, our research focuses on coding issues in IoT automation configuration, covering three categories: (1) implementing new features, (2) debugging, and (3) optimization.

% functional bugs in IoT automation configurations/implementations, instead of security issues.

He et al.~\cite{He2019} conducted an online survey with 72 users of smart home systems, to learn of their negative user experiences. The participants reported fears of breaking the system by writing their own programs, and struggles of diagnosing or recovering from system failures. Similarly, Makhshari and Mesbah~\cite{makhshari2021iot} did interviews and surveys with IoT developers; they also found testing and debugging as the major challenges faced by IoT developers. However, neither study examines any widely used smart home platform to characterize the bug patterns or fixing strategies, let alone to provide concrete actionable advices to tool builders for those platforms.
Our study is motivated by and complement both studies. %and compliment them. 
%Motivated by the observation that IoT developers had lots of difficulty creating smart home systems, we decided to focus on HA---one of the most popular smart home platforms---and characterized the bug patterns as well as fixing strategies.

% conducted an empirical security analysis of the smart-home programming platform SmartThings. They applied static code analysis to 499 SmartThings apps as well as 132 device handlers; they also crafted test cases to explore undocumented features of that platform. They discovered two intrinsic design flaws that lead to siginificant overprivilege in SmartApps. They also exploited framework design flaws to construct four proof-of-concept attacks. 

%Alrawi et al.~\cite{alrawi2019sok} performed a security evaluation of home-based IoT deployment. They proposed a methodology to analyze security properties for home-based IoT devices, systematically reviewed the literature using this methodology to understand attack techniques, mitigations, and stakeholders. They also evaluated the security properties of 45 devices by running existing tools. 

Brackenbury et al.~\cite{Brackenbury2019} focused on the trigger-action programming (TAP) model. They first systematized the temporal paradigms through which TAP systems could express rules, and then taxonomized 10 classes of TAP programming bugs. As with Brackenbury et al., we also characterized bugs related to the TAP model. However, because we mainly focused on the automation bugs in HA, our observations are not limited to bugs about the control logic (e.g., control flow, timing, and inaccurate user expectation). Our observations also characterized (1) bugs about formatting as well as program syntax, (2) developers' bug fixes, (3) recurring implementation requests, and (3) frequent optimization needs.

%They also conducted an online survey with 153 participants, and found that the presence of a bug made it harder for participants to 
% Furthermore, they conducted an online survey with 153 participants, who were asked to assess a series of pre-written TAP rules and half of the rules exhibited bugs. For most of the bug classes, the authors found that the presence of a bug made it harder for participants to correctly predict the behavior of the rule.  

Zhou et al.~\cite{Zhou2021} reviewed the 20 logic bugs mentioned for IoT systems and classified them. However, it is unknown on which platforms the bugs exist, and whether the list of bugs or categories are representative.
Wang et al.~\cite{wang2022understanding} inspected 330 device integration bugs mined from HAC to characterize any root cause, fix, trigger condition, and impact of those bugs. Our study is closest to the work by Wang et al., as we also examined data mined from HAC. However, we focused on the coding issues related to automation configurations, instead of device integration bugs.


\subsection{Automatic Bug Detection in IoT Systems}
Tools were created to automatically detect bugs in IoT systems~\cite{liang2016understanding,celik2018soteria,trimananda2020understanding,Li2020,Xiao2020,Fu2021,Huang2023}. 
Specifically, VulHunter~\cite{Xiao2020} detects vulnerabilities based on the known vulnerability patch packs in Industry IoT. SOTERIA~\cite{celik2018soteria} verifies whether IoT apps adhere to the identified safety, security, and functional properties via model checking.
Liang et al.~\cite{liang2016understanding} and Fu et al.~\cite{Fu2021} separately created tools to reveal bugs in IoT operating systems (OSes). 
%In particular, Liang et al.~inspected 23 fixed bugs in 3 IoT OSes, summarized 4 bug patterns, and created a rule-based bug detector accordingly. Fu et al.~created a tool CPscan, to identify bugs introduced by developers when they customized the Linux kernel via code pruning to create IoT kernels. CPscan compares the kernels before and after pruning, locates deleted security operations (DSO), and assesses the security impact. 

Some tools~\cite{trimananda2020understanding,Li2020,Huang2023} detect conflicting interactions between smart home IoT applications, because these conflicts can result in undesired actions like locking a door during a fire. For instance, Trimananda et al.~\cite{trimananda2020understanding} studied 198 official and 69 third-party apps on Samsung SmartThings, and found 3 major categories of app conflicts. Based on their observations, the researchers created a conflict detector that uses model checking to detect up to 96\% of the conflicts.
Li et al.~\cite{Li2020} categorized conflicts in a totally different way. They also invented a graph structure named \emph{IA graph} to represent the controls in each IoT app and event schedules. With that representation, they created an efficient algorithm to leverage first-order logic and SMT solvers to detect conflicts. 

Our study complements all tools mentioned above; it focuses on a different type of IoT bugs---bugs in automation configuration or implementation. Such implementation bugs are less relevant to security, IoT kernels, or inter-app conflicts. However, they are still important as these bugs can prevent end-users from realizing the desired automation rules or achieving high-quality automations.


%Fu et al.~created a tool to detect bugs in IoT kernels, which were customized by developers via removing code from the Linux kernel.
% studied 23 fixed bugs in 3 IoT operating systems (OSes): Contiki, TinyOS, and RIOT OS. Based on the root causes summarized for these 23 bugs, the researchers implemented a rule-based bug detector and successfully found previously unknown but later confirmed bugs in those OSes.
